Contact Surface Estimation via Haptic Perception

Legged systems need to optimize contact force in order to maintain contacts. For this, the controller needs to have the knowledge of the surface geometry and how slippery the terrain is. We can use a vision system to realize the terrain, but the accuracy of the vision system degrades in harsh weather, and it cannot visualize the terrain if it is covered with water or grass. Also, the degree of friction cannot be directly visualized. In this paper, we propose an online method to estimate the surface information via haptic exploration. We also introduce a probabilistic criterion to measure the quality of the estimation. The method is validated on both simulation and a real robot platform.

==> ext/tex/abbreviations.tex <==
\newcommand{\newabbreviation}[2]{#1\ (\renewcommand{#1}{#2}#1)}

% months
\newcommand{\jan      }{January}
\newcommand{\feb      }{February}
\newcommand{\mar      }{March}
\newcommand{\apr      }{April}
\newcommand{\may      }{May}
\newcommand{\jun      }{June}
\newcommand{\jul      }{July}
\newcommand{\aug      }{August}
\newcommand{\sep      }{September}
\newcommand{\oct      }{October}
\newcommand{\nov      }{November}
\newcommand{\dec      }{December}

% King's
\newcommand{\KCL    }{King's College London}
\newcommand{\NMS    }{Natural and Mathematical Sciences}
\newcommand{\CORE   }{the Centre for Robotics Research}
\newcommand{\RLL    }{Robot Learning Lab}
\newcommand{\WLab   }{Wheatstone Innovation Lab}

% Universities/research institutes
\newcommand{\TUM    }{Technische Universit\"{a}t Munich}
\newcommand{\MIT    }{Massachusetts Institute of Technology}

% funding bodies/schemes
\newcommand{\ERC    }{European Research Council}
\newcommand{\EPSRC  }{Engineering and Physical Sciences Research Council}
\newcommand{\CC     }{Crafts Council}
\newcommand{\JSPS   }{Japan Society for the Promotion of Science}
\newcommand{\AHDB   }{Agriculture and Horticultural Development Board}
\newcommand{\RSSB   }{Rail Safety and Standards Board}
\newcommand{\CONACYT}{Consejo Nacional de Ciencia y Tecnologia}
\newcommand{\HZOZO  }{Horizon 2020}
\newcommand{\FPZ    }{Seventh Framework Program}
\newcommand{\KTP    }{Knowledge Transfer Partnership}
\newcommand{\RIA    }{Research and Innovation Action}
\newcommand{\CTF    }{College Teaching Fund}

% journals, conferences
\newcommand{\TRo    }{IEEE Transactions on Robotics}
\newcommand{\TNSRE  }{IEEE Transactions on Neurorehabilitation Engineering}
\newcommand{\TMech  }{IEEE Transactions on Mechatronics}
\newcommand{\IJRR   }{International Journal of Robotics Research}
\newcommand{\NC     }{Neural Computation}
\newcommand{\AURO   }{Autonomous Robots}
\newcommand{\ICRA   }{IEEE International Conference on Robotics and Automation}
\newcommand{\IROS   }{IEEE International Conference on Intelligent Robots and Systems}
\newcommand{\RSS    }{Robotics: Science and Systems}
\newcommand{\Humanoids}{IEEE International Conference on Humanoid Robots}
\newcommand{\AIM    }{ASME/IEEE International Conference on Advanced Intelligent Mechatronics}
\newcommand{\ICORR  }{IEEE International Conference on Rehabilitation Robotics}
\newcommand{\BioRob }{IEEE International Conference on Biomedical Robotics and Biomechatronics}
\newcommand{\NIPS   }{Advances in Neural Information Processing Systems}

% people
\newcommand{\PI     }{principle investigator}
\newcommand{\CoI    }{co-investigator}
\newcommand{\PDRA   }{postdoctoral research assistant}
\newcommand{\UG     }{undergraduate}
\newcommand{\PG     }{postgraduate}
\newcommand{\TA     }{teaching assistant}
\newcommand{\MH     }{Matthew Howard}

% certificates/qualifications
\newcommand{\BSc}    {BSc}
\newcommand{\MSci}   {MSci}
\newcommand{\MSc}    {MSc}
\newcommand{\PhD}    {PhD}
\newcommand{\PGCAPHE}{Postgraduate Certificate in Academic Practice in Higher Education}

% machine learning
\newcommand{\RL     }{reinforcement learning}
\newcommand{\HMMs   }{hidden Markov models}

% robotics
\newcommand{\RAS    }{Robotics and autonomous systems}
\newcommand{\ROS    }{Robot Operating System}
\newcommand{\PbD    }{programming by demonstration}
\newcommand{\DoF    }{degrees of freedom}
\newcommand{\VIA    }{variable impedance actuator}
\newcommand{\EMG    }{electromyography}
\newcommand{\VPSA   }{variable physical stiffness actuator}
\newcommand{\CCL    }{constraint consistent learning}

% bibliographies
\newcommand{\Journal}{Journal}
\newcommand{\Eng    }{Engineering}
\newcommand{\Trans  }{Transactions}

% general
\newcommand{\WP     }{work package}
\newcommand{\TRL    }{technology readiness level}
\newcommand{\SMEs   }{small and medium enterprises}
\newcommand{\OA     }{open access}
\newcommand{\ICT    }{information and communication technology}
\newcommand{\HCI    }{human computer interfaces}



==> ext/tex/graphics.tex <==
% use graphicx for including images, set default image path
\usepackage{graphicx}
\graphicspath{{fig/}} 



==> ext/tex/meta.tex <==
\newcommand{\thetitle}         {}
\newcommand{\theshorttitle}    {}
\newcommand{\theauthor}        {Hsiu-Chin Lin}
\newcommand{\theshortauthor}   {H-C. Lin}


==> ext/tex/operators.tex <==
\usepackage{color}
\newcommand{\mh}[1]{\textcolor{red}{[MH: #1]}}
\definecolor{orange}{RGB}{255,128,0}
\newcommand{\todo}[1]{\textcolor{magenta}{(Todo:~#1)}}
\newcommand{\highlight}[1]{\textcolor{blue}{#1}}
\newcommand{\notes}[1]{\textcolor{orange}{(HC:~#1)}}
\renewcommand{\mh}[1]{}
\renewcommand{\todo}[1]{}


==> tex/notes.tex <==
\begin{equation}
\prob{\bD|\contactNormal} \sim \gaussianDist(\bZero, \gaussianCov) 
\end{equation}
\noindent 
where $\gaussianCov$ is the covariance matrix.


gives $\likelihood{\contactNormal_k|\bD}$ has a normal distribution $\contactNormal_k|\bD \sim \NormalDist{\mu}{\sigma}$
\[
 \prob{\contactNormal_k|\bD} \propto \prod_i^\dimPoints \prob{\contactNormal_k} \prob{\bx_i|\contactNormal}
\]
\noindent where $\sigma_x^2$ is the observation variance.

We would like to know what is the probability of the estimation $\contactNormal$.

\subsection{Problem Definition}

\noindent Let $\bp, \bpdot, \bpddot \in \R^{\dimFeet}$ denotes the position, velocities, and accelerations of the feet.
The joint space and end-effector space are related through %$\bq$ and $\bp$ are related through the kinematic map $\bp = \forwardKin(\bq)$ and 
%$\bqdot$ and $\bpdot$ are related through 
the Jacobian $\bpdot = \bJ(\bq)\bqdot$ and $\bpddot = \bJ(\bq)\bqddot + \bJdot \bqdot$.
We can consider that the constraint Jacobian can be described as 
\begin{equation}
 \bJ_c(\bq)  =  \bLambda \bJ(\bq) 
 \label{e:background-constraint-jacobian}
\end{equation}

\noindent 
where $\bLambda \in\R^{\dimFeet\times\dimFeet}$ is a set of normal or zero vectors that specifies which dimension is constrained.
Note that, $\bLambda$ does not need to be full rank and can contain only zeros in its rows.
When the robot is in contact with the surface, the contact surface acts as a constraint that restricts some of the motion.
From 
\begin{equation}
 \bJ_c \bqdot =\bZero
 \label{e:background-joint-constraint}
\end{equation}

\noindent 
Substitute \eref{background-constraint-jacobian} into \eref{background-joint-constraint}
\begin{equation}
 \bLambda \bJ(\bq) \bqdot =  \bLambda \bpdot =\bZero
 \label{e:background-constraint}
\end{equation}

\noindent 
From the above equation, if we can find the matrix $\bLambda$, so that we can construct $\bJ_c$.
The physical meaning is, we seek the direction of constraints such that the end-effector velocities in that direction is $\bZero$.


\begin{example} 
Assuming that the robot is moving over a flat terrain. The movement in z-axis is restricted since the feet cannot penetrated the surface. 
In this particular example, $\bpdot_z= 0$. the constraint Jacobian $\Jacobian_c$ would be a matrix that relates the joint velocities to the end-effector velocities along the z-axis.
\end{example}

